Indoor Scene Generation from a Collection of Semantic-Segmented Depth Images

We present a method for creating 3D indoor scenes with a generative model learned from a collection of semantic-segmented depth images captured from different unknown scenes. Given a room with a specified size, our method automatically generates 3D objects in a room from a randomly sampled latent code. Different from existing methods that represent an indoor scene with the type, location, and other properties of objects in the room and learn the scene layout from a collection of complete 3D indoor scenes, our method models each indoor scene as a 3D semantic scene volume and learns a volumetric generative adversarial network (GAN) from a collection of 2.5D partial observations of 3D scenes. To this end, we apply a differentiable projection layer to project the generated 3D semantic scene volumes into semantic-segmented depth images and design a new multiple-view discriminator for learning the complete 3D scene volume from 2.5D semantic-segmented depth images. Compared to existing methods, our method not only efficiently reduces the workload of modeling and acquiring 3D scenes for training, but also produces better object shapes and their detailed layouts in the scene. We evaluate our method with different indoor scene datasets and demonstrate the advantages of our method. We also extend our method for generating 3D indoor scenes from semantic-segmented depth images inferred from RGB images of real scenes.

==> contents/rebuttal.tex <==
% Pool: 1.1, 1.3, 1.4, 1.5, 2.1, 3.2, 3.3, 3.4, 3.5, 3.6
We thank the reviewers for their constructive comments. We will incorporate all of their suggestions in the revision and improve our writing. Also, we will release our code and model after the paper is published. 

% Try to respond 1.2/3.1
%We appreciate the reviewer's recognition of the key contribution of our work: learning a GAN model for 3D indoor scene layout generation from 2.5D semantic-depth images. Compared to other existing methods, our method needn't any complete 3D scene for training and generates better 3D scene layouts.  

\noindent\textbf{Our method vs. 3D-SLN (R1)}

We haven't realized any other methods for learning the generative model of 3D scene layouts from a collection of 2.5D scene images. The 3D-SLN (Luo, et al. End-to-end optimization of scene layout.CVPR20) work also requires the 3D complete scene dataset (SUNCG) for training a VAE model for scene layout generation. The 2.5D images are only used for refining the generated 3D scene layouts. In contrast, our method directly learns a GAN model of 3D scene layouts from 2.5D images. 

% Response 3.1
\noindent\textbf{Our method vs. HoloGAN[13] (R3, R2)}

Our method is different from HOLOGAN in several aspects. First, the HoloGAN tried to learn 3D object synthesis, while our method is designed for generating 3D scene layouts, which is "a harder task than object synthesis"(R3). Second, The HoloGAN represents objects with feature volumes. Without the disentangled representation of the objects' shape and appearance, it fails to generate a consistent projection of 3D objects under different poses. On the contrary, our method models the scene geometry and layouts as semantic volume, which guarantees consistent projection from different views. This is critical for learning 3D scene layouts from image collections randomly sampled from different 3D scenes. Finally, different from HoloGAN that applies a single discriminator in training, we proposed a multiple-view discriminator for our task. As discussed in Sec.4.3, the multiple view discriminator is not a trivial extension of the one used in HoloGAN but is carefully designed for 3D scene layout synthesis. We believe that our investigation behind this design (L410-L415 and the supplemental) is valuable to other GAN training and vision tasks.  

%via a is designed for learning a generative model of 3D objects, while our goal is to learn a GAN of 3D scene layout. we address a very different problem -- indoor scene generation rather than objects, leading to a more challenging task due to the camera and objects variant. To deal with it, we design a more complex but efficient multi-discriminator structure. Second, HoloGAN uses an implicit volume representation while we use an explicit one and regard the semantic volume as the final output. To achieve that, we use the DRC rather than RenderNet used in HoloGAN. To overcome the bias brought from the DRC, we design a novel view selection and multi-view aggregation strategy to make it work. We believe that our work is not a simple extension of HoloGAN but a novel exploration of indoor scene generation.

\noindent\textbf{Volumetric representation \& resolution (R1, R3)}
%Since the goal of this work is to model the object layout in a scene but not their detailed shapes, 

The semantic volume well models the rough object shapes(e.g. the sofa in Fig.5 [R1,C2] in the supplemental), which not only provides better input for shape retrieval (Fig.4), but also models the detailed layouts of the objects (e.g., Fig 7 [R1, C5/6]: chair under a desk; Fig.7 [R2, C3]: TV in TV stand) that are difficult to be modeled by the previous methods. Meanwhile, the semantic volume representation can be easily combined with differentiable projection for learning 3D scene layouts from semantic depth images. The low-resolution semantic volume $32\times32\times16$ achieves a good balance between model capability and computational cost. We trained the GAN model with $64\times64\times32$ volume resolution and the results are similar. 

  
%We agree that learning a GAN for generating both objects' layout and their detailed shapes is an interesting future work.        
% Not ready now, Since the goal of this work is to model the object layout in a scene but not their detailed shapes,

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/demonstrate}
%     \caption{Typical cases of non-cubic Manhattan layouts generated by our method. All cases are selected from the results shown in the paper and supplemental material.}
%     \label{FIG-NCM}
% \end{figure}
\noindent\textbf{Non-cubic Manhattan layout assumption (R1)} 

Thanks to the semantic volume representation, our method can learn "non-cubic Manhattan layouts" that are common in the real world (e.g. NYUv2 and MatterPort3D), such as the chair under a desk ([Row1, Column 4,5,6] of Fig.7), TV inside a TV cabinet ([R2, C1] of Fig.5), as well as the chairs with variant orientations ([R1, C1], [R2, C2] of Fig. 6 in the supplemental). Our method now assumes the room shape is cuboid but it can be easily extended for non-cuboid rooms.  


\noindent\textbf{More automated evaluations (R2)} 

We implemented the similarity metric in PlanIT[23]. The average similarity of the generated scene layouts and GT are $0.335$(Gen) and $0.457$(GT) respectively, which indicates that our method can generate variant scene layouts. We also followed the method in Fast\&Flexible[17] and evaluated the real vs. synthesis classification accuracy of our method by training a classifier with 800 semantic depth maps rendered from the generated scenes with random viewpoints and 800 GT semantic depth maps. After that, we computed the accuracy score with 320 rendered semantic depth maps and the result is $60.9\%$, which illustrates that our results are difficult to be classified as real or fake.

\noindent\textbf{Optimal view configuration \& camera pose (R3)} 

% Since we assume the GT images are captured from different scenes and we have no scene ID info of each image, we have no GT layout of each underline scene. We thus used a random combination of GT images captured from different scenes to approximate the layout of one underline scene. Our study in Sec.4.3 indicates that combinations with different number of images have different  and explored what kind of combination is a good approximation (Sec.4.3). If the object distribution of an image combination is different from the object distribution of the underline scenes, the generated scene may include too many or too few objects in specific category and thus     the object distribution  discussed how many GT images can provide a good approximation of scene layout, in which the object distribution offers a metric to measure the similarity of two scene layouts.  During GAN training, we followed the distribution of camera locations and poses of the training data to determine the camera location and poses of 4 views for projecting the generated scene volume. We did not put cameras at the center of the volume. 

Since we assume the GT images are captured from different scenes and we have no scene ID info of each image, we have no GT layout of each underline scene. We thus used a random combination of GT images captured from different scenes to approximate the layout of one underline scene. Sec.4.3 (L430-L485) discussed how many images in a combination can well approximate the layout of the underline scene (measured by the object distribution) and the optimal solution is 4. During GAN training, we do follow the view distribution of the GT images for projecting the synthesized scene volume and do not place the camera at the volume center. 

%The camera position and rotation, for generated scenes, are randomly selected and permutation-based on the distribution of the target dataset. The bias is from the DRC mechanism in the generative task with large depth variations in the training data (described in Sec.1 in the supplemental material). In the demonstration, we cancel the influence from the camera rotation and only consider the one from the camera position. Fig.1 in the supplemental material shows that the results will be biased to near views of independent discriminator design, while the proposed joint-discriminators design could fit the ground truth well. And for the number of views, we statistics the co-occurrence error with variant combinations of angel and number of views. For a common-used camera with about $100^\circ$ view coverage (statistics from Structured3D and Matterport3D), we select $4$ views per scene.

\noindent\textbf{Fair comparison with DeepPrior and GRAINS(R3)} 

We used the semantic depth maps rendered from the \emph{same SUNCG dataset} for a fair comparison with the prior works trained with SUNCG (L634-L638). We will clarify this in the revision.  

\noindent\textbf{Semantic maps from 2D semantic segmentation (R3)} 

Our method works well for semantic maps generated from 2D semantic segmentation. Specifically, for the unlabeled raw NYUv2 RGBD dataset, we discarded the depth maps and applied an existing RGB2depth network[12] to infer the depth and semantic maps from the RGB images and then trained the GAN model with the resulting semantic depth maps (L614-619). As shown in the last row of Fig.7 and the last three rows of Fig.6 in the supplemental, our method still generates reasonable 3D scene layouts. 
